Response to NITRD, NCO, NSF Request for Information on "Update to the 2016 National Artificial Intelligence Research and Development Strategic Plan"

We present a response to the 2018 Request for Information (RFI) from the NITRD, NCO, NSF regarding the "Update to the 2016 National Artificial Intelligence Research and Development Strategic Plan." Through this document, we provide a response to the question of whether and how the National Artificial Intelligence Research and Development Strategic Plan (NAIRDSP) should be updated from the perspective of Fermilab, America's premier national laboratory for High Energy Physics (HEP). We believe the NAIRDSP should be extended in light of the rapid pace of development and innovation in the field of Artificial Intelligence (AI) since 2016, and present our recommendations below. AI has profoundly impacted many areas of human life, promising to dramatically reshape society --- e.g., economy, education, science --- in the coming years. We are still early in this process. It is critical to invest now in this technology to ensure it is safe and deployed ethically. Science and society both have a strong need for accuracy, efficiency, transparency, and accountability in algorithms, making investments in scientific AI particularly valuable. Thus far the US has been a leader in AI technologies, and we believe as a national Laboratory it is crucial to help maintain and extend this leadership. Moreover, investments in AI will be important for maintaining US leadership in the physical sciences.

==> extras.tex <==

% Projects
% * neutrino reconstruction
% * FPGAs for fast inference and low power compute
% * HL-LHC reconstruction
% * accelerator controls
% * Cosmology/Astro
% ** telescope controls (scheduling)
% ** object classification and measurement; semantic segmentation (similar to reconstruction)
% ** multi-messenger analysis
% ** dedicated processors for fast analysis on future surveys?


% left-overs from the QC 

%The QC machines in use today (e.g. from Google, IBM, Rigetti, IonQ, etc.) all require specialized knowledge for how to set up and calibrate ``QC jobs'', run the jobs, and analyze the results. 

%A center will efficiently work with machine experts to acquire and disseminate such information and will need participation of classical computing experts, quantum computing experts, and HEP science and analysis experts. We believe that investing on such center(s) will result in transformational benefits for HEP, acting as the pole of attraction and a base of support for a user community at the labs and in academia with students and post-docs, thus it should be a central part of a HEP QIS R\&D program. Such center(s) will also be a catalyst for natural collaborations among lab personnel, industry machine expert partners, and faculty, post-docs and students from academia.


%\subsection{Fundamental Science Applications}
%Challenges we see: speed of data analysis; finding new ideas in such large data sets.
%Areas where these challenges exist. (Then what are the paths to solutions?)
%\begin{enumerate}
%\item particle physics
%\item cosmology and astrophysics: measurement and simulation (full multiwavelength data sets could revolutionize discovery space) of maps and objects
%\item theory (e.g., symmetry exploration) and hypothesis generation (new ideas and new science)
%\end{enumerate}

%\subsection{Improving AI Algorithms}
%Challenges we see: making AI ready for science; mixing AI with other algorithms and methods
%Areas where these challenges exist. (Then what are the paths to solutions?)
%    \begin{enumerate}
%        \item statistics and errors
%        \item implementation in QC environment
%        \item interpretability
%        \item scalability
%    \end{enumerate}

%Challenges we see: access to compute; sharing of data sets; structure for clearly comparing algorithms
%\subsection{Tools and Infrastructure}
%    \begin{enumerate}
%        \item industry writes the code {\color{red} NO! Industry write the \emph{frameworks} (e.g., TensorFlow), but many groups develop algorithms and applications}
%        \item hepcloud
%        \item integration with physics detection and instrumentation
%        \item Augmented Intelligence: allowing humans to use AI efficiently
%        \item data sharing (good niche for particle physics, maybe not for astro)
%        \item code comparison/housing/benchmarking
%        \item use AI to increase efficiencies in the work environment (energy usage, IT, )?
%        \item what about in an era when AI can be used to design new hardware. We should probably be thinking about hardware design if we're supposed to be creative and reach high.
%    \end{enumerate}

%\item Develop effective methods for human-AI collaboration.
%\begin{itemize}
%    \item We need improvements on merging standard tools with AI tools, and integrating AI tools into current workflows (or conversely evolving workflows to incorporate AI). \notes{We are relatively early adopters of the core technologies, and can help guide how AI systems and humans can complement each other, rather than AI systems full replacing us. This dovetails with the idea of workforce development.} 
%    \item {\color{blue}This could be an interesting avenue to look for industry partners - for example, how do we build a system that lets us ask natural language questions of our data? or a system we can interact with naturally to produce complex visualizations? Particle physics data analysis is extremely complex and could strongly benefit from such tools.}
%\end{itemize}

%\item Understand and address the ethical, legal, and societal implications of AI.
%\begin{itemize}
%\end{itemize}

\item Develop shared public datasets and environments for AI training and testing.

\begin{itemize}
    \begin{itemize}
        \item Cosmo: new, fast simulations: n-body and n-body + baryons are the new frontier for generative models.
        \item Cosmo: fast, fully automated analyses of imaging data; can help with optimizing follow-up of objects that will eventually disappear (e.g., multi-messenger astronomy and grav waves).
    \end{itemize}
\end{itemize}


\item Ensure the safety and security of AI systems.
\begin{itemize}
%\item We need to develop much stronger systems of algorithm explainability and accountability. \notes{(This utilizes HEP strengths in uncertainty quantification, error analysis, etc. - this is also how we support reconstruction efforts, by moving beyond vision and into semantic understanding, etc.)}
\item {\color{blue}Important for a controls project - how to build \emph{real time} safeguards \cite{7454846}.}
\item {\color{blue}Other points? - should we talk to FNAL security people about what they are thinking about here (there is some work on systems for defeating CAPTCHAs at FNAL, etc.)}
\end{itemize}

